Chaotic Properties of the Elliptical Stadium

The elliptical stadium is a curve constructed by joining two half-ellipses, with half axes a>1 and b=1, by two straight segments of equal length 2h. In this work we find bounds on h, for a close to 1, to assure the positiveness of a Lyapunov exponent. We conclude that, for these values of a and h, the elliptical stadium billiard mapping is ergodic and has the K-property.

==> fig2.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       9.75       2.84 {$\scriptstyle\varphi_0$                                                         }
\point       9.01       3.05 {$\scriptstyle\theta_0$                                                          }
\point       7.99       4.26 {$\scriptstyle\varphi_1$                                                         }
\point       7.29       3.78 {$\scriptstyle\theta_1$                                                          }
\point       5.49       3.64 {$\scriptstyle\varphi_2$                                                         }
 }}


==> fig3.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point      12.12       0.80 {$a$                                                                             }
\point       0.92       0.40 {$\sqrt{4 - 2 \sqrt{2}}$                                                         }
\point       2.95       0.40 {$2\sqrt{3}/3$                                                                   }
\point       4.81       0.40 {$\sqrt{2}$                                                                      }
\point       7.09       0.40 {$2$                                                                             }
\point       8.83       0.40 {$\sqrt{4 + 2\sqrt{2}}$                                                          }
\point      12.25       1.71 {$\tau = 1/4$                                                                    }
\point      12.25       3.04 {$\tau = 1/3$                                                                    }
\point      12.25       4.37 {$\tau = 1/2$                                                                    }
\point      12.25       5.71 {$\tau = 2/3$                                                                    }
\point      12.25       7.04 {$\tau = 3/4$                                                                    }
\point      12.25       1.97 {$period\ 8$                                                                     }
\point      12.25       3.31 {$period\ 6$                                                                     }
\point      12.25       4.64 {$period\ 4$                                                                     }
\point      12.25       5.97 {$period\ 6$                                                                     }
\point      12.25       7.31 {$period\ 8$                                                                     }
 }}


==> fig4.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       7.05       2.67 {$2h$                                                                            }
\point       8.69       1.58 {$a$                                                                             }
\point       8.43       1.86 {$1$                                                                             }
 }}


==> fig5.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{\small
\point       6.53       4.78 {$\theta$             }
\point       6.80       0.33 {$ 0$                 }
\point       8.90       0.33 {$ \pi$               }
\point       9.60       0.33 {$ \pi + 2h$          }
\point      11.55       0.33 {$ 2\pi+2h$           }
\point      13.30       0.67 {$\varphi$            }
\point       6.10       2.75 {$\varphi_0$          }
\point       8.10       2.86 {$\varphi_0$          }
\point       1.19       3.32 {$\varphi_1$          }
\point      10.10       2.32 {$\varphi_1$          }
 }}

